Tokenizer Choice For LLM Training: Negligible or Crucial?

The recent success of Large Language Models (LLMs) has been predominantly driven by curating the training dataset composition, scaling of model architectures and dataset sizes and advancements in pretraining objectives, leaving tokenizer influence as a blind spot. Shedding light on this underexplored area, we conduct a comprehensive study on the influence of tokenizer choice on LLM downstream performance by training 24 mono- and multilingual LLMs at a 2.6B parameter scale, ablating different tokenizer algorithms and parameterizations. Our studies highlight that the tokenizer choice can significantly impact the model's downstream performance and training costs. In particular, we find that the common tokenizer evaluation metrics fertility and parity are not always predictive of model downstream performance, rendering these metrics a questionable proxy for the model's downstream performance. Furthermore, we show that multilingual tokenizers trained on the five most frequent European languages require vocabulary size increases of factor three in comparison to English. While English-centric tokenizers have been applied to the training of multi-lingual LLMs in the past, we find that this approach results in a severe downstream performance degradation and additional training costs of up to 68%, due to an inefficient tokenization vocabulary.

==> preprocessing.tex <==
\subsection{Preprocessing}
We incorporate different high-quality datasets and 
For OSCAR the \emph{ungoliant} pipeline was used \cite{abadji_ortiz_etal2021} to prepare data from CommonCrawl datasets. The metadata provided by CommonCrawl are kept and were used for filtering the data based on quality warnings.
RedPajama published a 1 trillion token dataset from which we used the wikipedia subdataset. %

Our preprocessing pipeline consists of
\begin{enumerate}
    \item combining the various data sources
    \item filtering by OSCAR quality warnings and harmful perplexity
    \item deduplication using MinHashLSH
    \item shuffling
\end{enumerate}

Notes:

Jana:
RP: wikipedia etc. (JG+L)
- Wiki: The preprocessing applied by RedPajama on the Wikipedia Dataset covers the removal of hyperlinks and templates. \cite{redpajama2023}
- ArXiv: "We only keep latex source files and remove preambles, comments, macros and bibliographies."
- StackExchange: "we only keep the posts from the 28 largest sites, remove html tags, group the posts into question-answer pairs, and order answers by their score"


Hammam:
Pile: pile corpora describe preprocessing steps per dataset
- for all datasets: language clf
- PhilPapers: "we discard any papers with less than 1000 char-
acters", "papers with non-machine readable
text are ignored"
- OpenWebText2: URL-based dedup, "URLs with an aggregate score of less
then 3 were removed", further (MinHash) Dedup
- NIH Exporter: "Entries were deduplicated based off their
application ID, and excluded if their abstract text
was missing or too short. Small grants, especially
administrative ones, consisted solely of short boil-
erplate. For this reason, we further deduplicated on
abstract text"
- FreeLaw: /
- PMC Extracts: "we remove any
line beginning with :::, which is used by pandoc
to indicate html classes in markdown."
- PMC Abstracts: "contained a malformed title or abstract
and were excluded", "removed any copyright information.", removed any abstarcts already present in PMC


Lennard:
oscar: Ungoliant preprocessing steps for OSCAR (JG+L)
filtering: harmful pp(5,why?) (refer to paper), quality warnings>, (JG+L)
describe preprocessing for oscar and other data (JG+L)

quality warnings:
-tiny: The document has a low (<5) number of lines.
- short sentences: The document has a high number (>50%
- header: The document has a high number of short lines at its head, suggesting the presence of low quality content.
- footer: The document has a high number of short lines at its tail, suggesting the presence of low quality content.
- noisy: The document has a high percentage of punctuation (>50%
- adult: The document contains adult content. This annotation uses a blocklist and labels a tiny part of the corpus: It does not catch most of the adult content.

- harmful ppl: KenLM-based adult content detection (ppl), the lower it is, the more likely a given document contains harmful/adult content.
- (lang id)



==> tokenizer_params.tex <==
HuggingFace - BPE:
 - dropout
 - continuing subword prefix (The prefix to attach to subword units that don't represent a beginning of word)
 - end of word suffix (The suffix to attach to subword units that represent an end of word)
 - fuse unk (Whether to fuse any subsequent unknown tokens into a single one)
 - byte fallback (Whether to use spm byte-fallback trick)
 
 HuggingFace - BPE-Trainer:
 - min frequency (The minimum frequency a pair should have in order to be merged)
 - limit alphabet (The maximum different characters to keep in the alphabet)
 - continuing subword prefix (A prefix to be used for every subword that is not a beginning-of-word)
 - end of word suffix (A suffix to be used for every subword that is an end-of-word)
 
 SentencePiece:
 
 - accept language (comma-separated list of languages this model can accept)
 - self test sample size (the size of self test samples)
 - character coverage (character coverage to determine the minimum symbols) 
 - input sentence size (maximum size of sentences the trainer loads) 
 - shuffle input sentence (Randomly sample input sentences in advance)
 - seed sentencepiece size (the size of seed sentencepieces)
 - shrinking factor (Keeps top shrinking factor pieces with respect to the loss)
 - num sub iterations (number of EM sub-iterations)
 - max sentencepiece length (maximum length of sentence piece)
 - max sentence length (maximum length of sentence in byte)
 - split by unicode script (use Unicode script to split sentence pieces)

